IllinoisSL: A JAVA Library for Structured Prediction

IllinoisSL is a Java library for learning structured prediction models. It supports structured Support Vector Machines and structured Perceptron. The library consists of a core learning module and several applications, which can be executed from command-lines. Documentation is provided to guide users. In Comparison to other structured learning libraries, IllinoisSL is efficient, general, and easy to use.

==> conclusion.tex <==
\iSL is an open-source Java library for structured prediction. The library provides a simple, easy-to-use interface for ML practitioners
to train on large and complex data.
%The library has been used in many research projects and performs well. 
%The goal of \iSL is to provide a general platform for training large and complex data. 

 

